One-Shot Synthesis of Images and Segmentation Masks

Joint synthesis of images and segmentation masks with generative adversarial networks (GANs) is promising to reduce the effort needed for collecting image data with pixel-wise annotations. However, to learn high-fidelity image-mask synthesis, existing GAN approaches first need a pre-training phase requiring large amounts of image data, which limits their utilization in restricted image domains. In this work, we take a step to reduce this limitation, introducing the task of one-shot image-mask synthesis. We aim to generate diverse images and their segmentation masks given only a single labelled example, and assuming, contrary to previous models, no access to any pre-training data. To this end, inspired by the recent architectural developments of single-image GANs, we introduce our OSMIS model which enables the synthesis of segmentation masks that are precisely aligned to the generated images in the one-shot regime. Besides achieving the high fidelity of generated masks, OSMIS outperforms state-of-the-art single-image GAN models in image synthesis quality and diversity. In addition, despite not using any additional data, OSMIS demonstrates an impressive ability to serve as a source of useful data augmentation for one-shot segmentation applications, providing performance gains that are complementary to standard data augmentation techniques. Code is available at https://github.com/ boschresearch/one-shot-synthesis

==> figures/qual_results.tex <==
\begin{figure*}[t]
\begin{centering}
\setlength{\tabcolsep}{0.0em}
\par\end{centering}
\renewcommand{\arraystretch}{0.50}

\begin{tabular}{@{\hskip -0.05in}c@{\hskip -0.02in}c@{\hskip 0.024in}c@{\hskip 0.024in}c@{\hskip 0.024in}c@{\hskip 0.024in}c@{\hskip 0.056in}c@{\hskip 0.056in}c@{\hskip 0.024in}c@{\hskip 0.024in}c@{\hskip 0.024in}c@{\hskip 0.024in}}

& & \multicolumn{4}{c}{\small Generated samples} & & \multicolumn{4}{c}{\small Generated samples}
\tabularnewline

\multirow{-1}{*}{\begin{tabular}{c}  \small{Training pair} \\\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/00000.jpg} \\ \includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/00000_mask.jpg} \end{tabular}} &
\multirow{1}{*}{ \rotatebox{90}{MCA (ours) \hspace{-2.7em} }} &

\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/ours/12_im} & 
\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/ours/19_im} & 
\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/ours/0_im} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/ours/6_im} & 
	\multirow{1}{*}{ \rotatebox{90}{ Input concat. \hspace{-2.9em} }} &
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/concat/1_im} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/concat/3_im} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/concat/4_im} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/concat/9_im}  
	\tabularnewline \vspace{0.5ex}
	& &
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/ours/12_ma} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/ours/19_ma} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/ours/0_ma} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/ours/6_ma} & &
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/concat/1_ma} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/concat/3_ma} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/concat/4_ma} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/concat/9_ma} 
	\tabularnewline 
	
	& \multirow{1}{*}{ \rotatebox{90}{Projection \cite{miyato2018cgans} \hspace{-3.4em} }} &
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/projection/8_im} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/projection/18_im} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/projection/1_im} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/projection/53_im} & 
	\multirow{1}{*}{ \rotatebox{90}{ SemanticGAN \cite{li2021semantic} \hspace{-4.2em} }} &
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/semantic/3_im} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/semantic/6_im} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/semantic/11_im} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/semantic/33_im} \tabularnewline
	
	& &
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/projection/8_ma} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/projection/18_ma_2} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/projection/1_ma} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/projection/53_ma} &   &
	\includegraphics[width=0.099\linewidth, height=0.0614\textheight]{figures/qual_results/car/semantic/3_ma} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/semantic/6_ma} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/semantic/11_ma} & 
	\includegraphics[width=0.099\linewidth, height=0.06\textheight]{figures/qual_results/car/semantic/33_ma}
	\tabularnewline \tabularnewline


%\multirow{-1}{*}{\begin{tabular}{c}  \small{Training pair} \\\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/00000.jpg} \\ \includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/0_mask_sat.jpg} \end{tabular}} &
%\multirow{1}{*}{ \rotatebox{90}{MCA (ours) \hspace{-2.7em} }} &

%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/00000.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/00000.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/00000.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/00000.jpg} & 
%\multirow{1}{*}{ \rotatebox{90}{ Input concat. \hspace{-2.9em} }} &
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/00000.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/00000.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/00000.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/00000.jpg}
%\tabularnewline \vspace{0.5ex}
%& &
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/0_mask_sat.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/0_mask_sat.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/0_mask_sat.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/0_mask_sat.jpg} & &
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/0_mask_sat.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/0_mask_sat.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/0_mask_sat.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/0_mask_sat.jpg} 
%\tabularnewline  

%& \multirow{1}{*}{ \rotatebox{90}{Projection \cite{miyato2018cgans} \hspace{-3.4em} }} &
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/00000.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/00000.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/00000.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/00000.jpg} & 
%\multirow{1}{*}{ \rotatebox{90}{ SemanticGAN \cite{li2021semantic} \hspace{-4.2em} }} &
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/00000.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/00000.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/00000.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/00000.jpg} 
%\tabularnewline 

%& &
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/0_mask_sat.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/0_mask_sat.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/0_mask_sat.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/0_mask_sat.jpg} &  &
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/0_mask_sat.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/0_mask_sat.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/0_mask_sat.jpg} & 
%\includegraphics[width=0.10\linewidth, height=0.06\textheight]{figures/teaser/0_mask_sat.jpg}




\end{tabular}


\caption{Description.}
\label{fig:qual_results_comp}
\end{figure*}

==> figures/teaser_old.tex <==
\begin{figure}[t]

\includegraphics[width=1.0\linewidth]{figures/teaser/bild11}

\caption{
Given a single image and its pixel-level semantic annotation, our model can generate a diverse set of labelled images. The generated scenes exhibit a remarkable structural diversity, varying the locations of foreground objects and changing the layout of the background, while the produced segmentation masks achieve a good alignment to the layouts of synthetic images.
%Given a single image and its pixel-level semantic annotation, our SIV-GAN$_{\text{mask}}$ can produce diverse versions of the same scene, supplemented with high-fidelity label masks. Thanks to a high structural diversity among samples and to the good alignment between the masks and image content, such synthetic data can serve as data augmentation and bring additional performance gains to various one-shot semantic segmentation applications.\anna{1. method name - SIV-GANmask needs to be updated; 2. if we would go for image-mask synthesis pitch, the teaser figure needs to be changed; 3. also for the task of augmentation, showing doubled same instances might be counter intuitive, as the task here to track the unique object, while duplicating it results in the 2 instances, this might result in the questions from the reviewers, so I would pick another images
}
\label{fig:teaser}
\end{figure}



==> tables/archiv_exps.tex <==
\newpage  %% other old

\subsection{Evaluation Setup.}
\label{sec:exp-setup}

\myparagraph{GAN synthesis evaluation.} Evaluating the realism of synthetic images in the one-shot regime is changing, because the commonly used image quality metrics favour overfitting, penalizing deviations from the original sample \cite{sushko2021learning, robb2021fewshot, li2020few}. Thus, following \cite{sushko2021learning} we mind a possible quality-diversity trade-off, reporting SIFID \cite{Shaham2019SinGANLA} and LPIPS \cite{zhang2018unreasonable} to measure both the quality and diversity of image synthesis.

Evaluating the quality of generated masks is also not straightforward, as synthetic images do not have ground truth annotations. To bypass this issue, we propose to train an external segmentation network on the generated image-mask pairs and test its mIoU performance on the original real pair, augmented with standard geometric transformations. Intuitively, the good performance on this test reveals that synthetic data generalizes well to the real data, indicating the good alignment between the generated images and masks. We choose a simple UNet \cite{Ronneberger2015UNetCN} architecture for the segmenter, training it for 500 epochs.

\myparagraph{One-shot video object segmentation.} We apply our augmentation pipeline to the semi-supervised 
one-shot video segmentation benchmark DAVIS\footnote{https://davischallenge.org/}. At test time,  this setup provides a video and the semantic annotation of objects only in the first frame, while the models are required to segment all the remaining video frames. We conduct experiments on two DAVIS splits: \textit{DAVIS-16}, having 20 videos, with a single annotated object; and its extension \textit{DAVIS-17} which adds 10 new videos and introduces multi-instance annotations.
The images are generated at the resolution of 384x640 and then resized to the original resolution of 480x854. 
In this work, we experiment with two popular networks from the literature: 
\begin{itemize}
	\item \textbf{OSVOS} \cite{Cae+17}, a fully-convolutional approach leveraging the knowledge extracted from DAVIS training set and ImageNet \cite{imagenet_cvpr09}. At test time, the model fine-tunes the weights on the first frame, using data augmentation, and then processes the remaining video frames separately, without considering their temporal relation. 	For OSVOS, we add the selected synthetic samples to each fine-tuning batch before applying standard image augmentation, keeping the 50\%-50\% ratio between real and fake data.
	
	\item \textbf{STM} \cite{oh2019video}, an encoder-decoder network with a space-time memory block, allowing to efficiently utilize temporal relations between the test video frames. At inference, the model scans the test sequence frame-by-frame, updating the space-time memory with newly segmented frames. For STM, to fit the GPU memory limitations, we further restrict the amount of augmentations to 10 randomly picked synthetic examples. In order not to permute the temporal order of frames, the samples are appended to the memory bank at the zero step, before the first frame.
\end{itemize}

For the downstream video object segmentation performance, we report the mIoU region similarity ($\mathcal{J}$) and contour accuracy ($\mathcal{F}$), the two metrics commonly used in the literature on this task \cite{pont20172017}. 

\myparagraph{One-shot semantic image segmentation.} Next, we evaluate our pipeline on the public one-shot image segmentation benchmark COCO-20$^i$ \cite{Lin2014MicrosoftCC}. This dataset has 80 classes, which are divided into 4 folds with 60 base and 20 test classes in each fold. During training, a one-shot segmentation model extracts knowledge from the base classes. At inference, the model is given a single image-mask pair (support set) depicting an object of a previously unseen test class, and after that is required to segment another sample (query image) containing instance of the same class. The performance on this task is evaluated using mIoU across all test classes. 

We conduct experiments with the state-of-the-art RePRI network \cite{boudiaf2021few}. RePRI is trained on base classes using standard cross-entropy loss, bypassing episodic meta-learning commonly used in few-shot approaches. At test time, the network adapts to a given support sample with the introduced transductive inference scheme. 

We add our images...

Image resolution 417x417.
We test 100x4 images, use only a single class in each image. 

At inference, we add 10 images as augmentations of support set. 


\subsection{Results.}
\label{sec:exp-mainresults}

\myparagraph{Qualitative synthesis results.}
\vadim{here highlight structural diversity}

\myparagraph{Performance as data augmentation.}

\vadim{mention here that we average across 5. Define standard data augmentation.}
To account for the variance between runs, we average out the metrics across 5 repeated runs.

\subsection{Ablations.}
\label{sec:exp-ablations}

\vadim{here describe both table 3 and table 4}

\subsection{Comparison of MCA to other mask synthesis supervision methods.}
\label{sec:exp-comparison}










\newpage

%%%%%%%%% old


We extensively evaluate our proposed synthetic data augmentation pipeline as follows. Firstly, we assess the synthesis properties of the proposed model both qualitatively and quantitatively, showing its higher performance compared to the baselines (Sec. \ref{sec:exp-synthesis}). Next, we demonstrate the successful application of the generated samples to one-shot video object segmentation (Sec. \ref{sec:exp-app_video})  and one-shot semantic image segmentation (Sec. \ref{sec:exp-app_image}). Finally, we provide an ablation study to highlight the importance of the proposed technical contribution and the training data filtering (Sec. \ref{sec:exp-ablations}).




\subsection{Evaluation of the synthesis quality and diversity.}
\label{sec:exp-synthesis}

\myparagraph{Baselines.} We compare our Masked Content Attention with alternative mechanisms for the discriminator to provide supervision for the generator's label synthesis branch. The simplest baseline is to concatenate the input masks to images, when the discriminator is required to produce its decision based on the joint image-mask distribution. Another method is to use projection \cite{miyato2018cgans}, by taking the inner product between the last linear layer output of $D_{\text{low-level}}$ and the embedded mask. Finally, we compare to the approach of SemanticGAN \cite{li2021semantic}, using an additional $L_m$ discriminator taking both images and masks as input, and propagating gradients only to the label synthesis branch. All the baselines differ from the MCA, as they use the mask only as input, not in the loss function. While training all the baseline methods, we do not use the MCA, while preserving all the other training details. 

\myparagraph{Metrics.} Evaluating the realism of synthetic images in the one-shot regime is changing, because the commonly used image quality metrics favour overfitting, penalizing deviations from the original sample \cite{sushko2021learning, robb2021fewshot, li2020few}. Thus, following \cite{sushko2021learning} we mind a possible quality-diversity trade-off, reporting SIFID \cite{Shaham2019SinGANLA} and LPIPS \cite{zhang2018unreasonable} to measure both the quality and diversity of image synthesis.

Evaluating the quality of generated masks is also not straightforward, as synthetic images do not have ground truth annotations. To bypass this issue, we propose to train an external segmentation network on the generated image-mask pairs and test its mIoU performance on the original real pair, augmented with standard geometric transformations. Intuitively, the good performance on this test reveals that synthetic data generalizes well to the real data, indicating the good alignment between the generated images and masks. We choose a simple UNet \cite{Ronneberger2015UNetCN} architecture for the segmenter, training it for 500 epochs.



\myparagraph{Datasets and training details.} For the synthesis evaluation, we take the DAVIS \cite{pont20172017} dataset. For each video from the DAVIS-17 validation split, we take the first frame and its semantic label map, which results in 30 image-mask pairs which we use for training. In line with \cite{sushko2021learning} we evaluate the synthesis at the resolution of 192x320. We preserve all the training hyperparameters from \cite{sushko2021learning}, but extend the Differentiable Augmentation (DA) pipeline \cite{Karras2020TrainingGA}, as we found this step to improve both the quality and diversity of images (see Table \ref{tab:ablations}). We train the models for 150k epochs and select the checkpoints by SIFID. In this subsection, we do not use the data selection described in \ref{sec:method-selection}.
 



\myparagraph{Results.} 
The visual comparison to the baselines is presented in Fig. \ref{fig:qual_davis}. For our model, we remark a high structural diversity among samples and a high quality of generated annotations. For example, \vadim{here goes explanation of 1-2 images in Fig. DAVIS}. In contrast, the baselines cannot simultaneously achieve good quality, diversity, and precise alignment of masks annotations. Particularly, \textit{Input concatenation} leads to decreased diversity, as the generated images generally remind simple geometric augmentations of the training sample. The \textit{label projection} yields unstable training, leading to corruptions in the generated masks. An additional discriminator, as in \textit{SemanticGAN}, achieves comparable results to CMA, but has a disadvantage of computational overhead introduced by an extra network for training. 

The quantitative comparison is presented in Table \ref{tab:synthesis_evaluation}. Compared to the plain model without the mask synthesis mechanism, the Masked Content Attention helps to additionally regularize the discriminator, reducing memorization and achieving notably higher diversity (LPIPS of xx.x vs yy.y), without compromising image quality (SIFID of xx.x vs yy.y). In contrast, all the baseline methods affect the diversity negatively. 
Besides improved diversity, MCA achieves the best alignment of the generated masks to the image content, as measured by the trained UNet (highest mIoU of xx.xx in Table \ref{tab:synthesis_evaluation}).
In Sec. \ref{sec:exp-ablations} we demonstrate that a diverse image synthesis of our model, coupled with mask annotations of the highest quality, yields the best improvement when applied as data augmentation to one-shot video object tracking.

\subsection{Application to one-shot video object segmentation.}
\label{sec:exp-app_video}

We apply our augmentation pipeline to the semi-supervised one-shot video segmentation benchmark DAVIS\footnote{https://davischallenge.org/}. At test time,  this setup provides a video and the semantic annotation of objects only in the first frame, while the models are required to segment all the remaining video frames. In this work, we experiment with two popular networks from the literature: 

\begin{itemize}
	\item \textbf{OSVOS} \cite{Cae+17}, a fully-convolutional approach leveraging the knowledge extracted from DAVIS training set and ImageNet \cite{imagenet_cvpr09}. At test time, the model fine-tunes the weights on the first frame, using data augmentation, and then processes the remaining video frames separately, without considering their temporal relation. 	
	\item \textbf{STM} \cite{oh2019video}, an encoder-decoder network with a space-time memory block, allowing to efficiently utilize temporal relations between the test video frames. At inference, the model scans the test sequence frame-by-frame, updating the space-time memory with newly segmented frames.
\end{itemize}

We generate $N=100$ augmentations of the first frame and apply the data selection described in \ref{sec:method-selection}. The images are generated at the resolution of 384x640 and then resized to the original resolution of 480x854. For OSVOS, we add the selected synthetic samples to each fine-tuning batch before applying standard image augmentation, keeping the 50\%-50\% ratio between real and fake data. For STM, to fit the GPU memory limitations, we further restrict the amount of augmentations to 10 randomly picked synthetic examples. In order not to permute the temporal order of frames, the samples are appended to the memory bank at the zero step, before the first frame.

We conduct experiments on two DAVIS splits: \textit{DAVIS-16}, having 20 videos, with a single annotated object; and its extension \textit{DAVIS-17} which adds 10 new videos and introduces multi-instance annotations. For the downstream video segmentation performance, we report the mIoU region similarity ($\mathcal{J}$) and contour accuracy ($\mathcal{F}$), the two default metrics used in the literature \cite{pont20172017}. To account for the variance between runs, we average out the metrics across 5 repeated runs.

The results are presented in Table \ref{tab:results_video}. Our pipeline visibly improves the performance of both OSVOS and STM. Compared to the plain models without data augmentation, we measure an average absolute improvement of x.x $\mathcal{J}$ and y.y $\mathcal{F}$ across the two data splits.
In relative terms, this corresponds to bringing the $\mathcal{J}$ and $\mathcal{F}$ scores on average closer to the absolute performance of 100.0 by impressive x.x\% and y.y\%. 

Interestingly, the synthetic augmentations frequently outperform standard geometric transformations (lines 2-3 in Table \ref{tab:results_video}), indicating higher effectiveness of the structural diversity contained in GAN-generated samples. Moreover, we observe that the synthetic augmentation is complementary to the standard pipeline, as the highest performance is achieved when two augmentation pipelines are used in combination (last line in Table \ref{tab:results_video}).

In Fig. \ref{fig:viseo_sequences} we demonstrate the effect of synthetic augmentation added to the standard OSVOS pipeline on DAVIS-16. GAN-based samples improve the $\mathcal{J}$ for the vast majority of video sequences (x/20), with the most notable increase commonly achieved for the hardest video sequences.

\subsection{Application to one-shot semantic image segmentation.}
\label{sec:exp-app_image}

Next, we evaluate our pipeline on the public one-shot image segmentation benchmark COCO-20$^i$ \cite{Lin2014MicrosoftCC}. This dataset has 80 classes, which are divided into 4 folds with 60 base and 20 test classes in each fold. During training, a one-shot segmentation model extracts knowledge from the base classes. At inference, the model is given a single image-mask pair (support set) depicting an object of a previously unseen test class, and after that is required to segment another sample (query image) containing instance of the same class. The performance on this task is evaluated using mIoU across all test classes. 

We conduct experiments with the state-of-the-art RePRI network \cite{boudiaf2021few}. RePRI is trained on base classes using standard cross-entropy loss, bypassing episodic meta-learning commonly used in few-shot approaches. At test time, the network adapts to a given support sample with the introduced transductive inference scheme. 

We add our images...

Image resolution 417x417.
We test 100x4 images, use only a single class in each image. 
Which network we use.

At inference, we add 10 images as augmentations of support set. 

Results: over all splits, we see consistent improvement. Also complementary with data augmentation.


\subsection{Ablations.}
\label{sec:exp-ablations}

\vadim{here 1) compare synthesis quality - diversity - mIoU on applications with comparison baselines. AND same with loss balancing, DA or other design choices (are there any more?). 2) Rejection sampling ablation - importance of both quality and diversity. + ablate SIFID at different layers + ablate rejecting by mIoU mask (should be not beneficial compared to SIFIDs) }


==> tables/joint_synthesis.tex <==
\begin{table*}[t]
\centering


\begin{minipage}{.33\linewidth}
	
%\setlength{\tabcolsep}{0.50em}
\renewcommand{\arraystretch}{1.20}
%\centering
%\centering	
%@{\hskip 0.02in}
\centering
\caption{Comparison of the image synthesis quality and diversity to previous methods on DAVIS-17. Bold denotes the best performance.}
\label{table:ablations} %
\begin{tabular}{@{\hskip 0.03in}l@{\hskip 0.03in}|@{\hskip 0.03in}c@{\hskip 0.03in}|@{\hskip 0.03in}c@{\hskip 0.03in}}
	
	\multirow{2}{*}{Method} & \multirow{2}{*}{SIFID$\downarrow$}  & \multirow{2}{*}{LPIPS$\uparrow$} % & \multirow{2}{*}{mIoU$_\text{mask}$$\uparrow$} 
	\tabularnewline 
	& & \tabularnewline
	
	\hline 	
	
	SinGAN \cite{Shaham2019SinGANLA} & 0.131 & 0.267 %  & - 
	\tabularnewline
	ConSinGAN \cite{Hinz2020ImprovedTF} & 0.103 & 0.296 %  & - 
	\tabularnewline \arrayrulecolor{lightgray}	\hline \arrayrulecolor{black}
	% \arrayrulecolor{lightgray} \hline \arrayrulecolor{black}
	One-Shot GAN \cite{sushko2021learning} & 0.091 & 0.347 % & - 
	\tabularnewline 		
	~~+ improved DA & \textbf{0.071} & 0.368 % & - 
	%		\tabularnewline
	%		~~+ ours, w/o $\{\alpha_i\}$  & 0.068 & 0.381 & 91.9 
	\tabularnewline \arrayrulecolor{lightgray}	\hline \arrayrulecolor{black}
	OSMIS (ours) & 0.073 & \textbf{0.387} % & \textbf{92.6} 
	%		\tabularnewline
\end{tabular}
	
\end{minipage}
% -------------------------------------------------------------------
\begin{minipage}{.43\linewidth}
		
\caption{Comparison of MCA to other label synthesis supervision mechanisms on DAVIS-17. 
Red indicates decreased diversity compared to the baseline. Bold denotes the best performance.}
\label{table:comparison} %

%\setlength{\tabcolsep}{0.50em}
\renewcommand{\arraystretch}{1.20}
%\centering
	
%@{\hskip 0.02in}
\centering
\begin{tabular}{@{\hskip 0.03in}l@{\hskip 0.03in}|@{\hskip 0.03in}c@{\hskip 0.03in}|@{\hskip 0.03in}c@{\hskip 0.03in}|@{\hskip 0.03in}c@{\hskip 0.03in}}
	%& \multicolumn{3}{c||@{\hskip 0.03in}}{\scriptsize \color{black} Synthesis quality} % & \multicolumn{2}{c}{\scriptsize \color{black} Effect on  performance}
	%\tabularnewline		
	
	\multirow{2}{*}{Mask supervision} & \multirow{2}{*}{SIFID$\downarrow$}  & \multirow{2}{*}{LPIPS$\uparrow$} & \multirow{2}{*}{mIoU$_\text{mask}$$\uparrow$} % & \multicolumn{2}{c}{\scriptsize \color{black} of OSVOS \cite{Cae+17}}
	\tabularnewline
	
	& &  & % & $\mathcal{J}$ & $\mathcal{F}$ 
	\tabularnewline	
	\hline 	
	
	None & 0.071 & 0.368  & -  % & \color{gray} 76.7 \scriptsize{(+0.0)} & \color{gray} 80.2 \scriptsize{(+0.0)} 
	\tabularnewline 
	\arrayrulecolor{lightgray}	\hline \arrayrulecolor{black}
	Projection \cite{miyato2018cgans} & \textbf{0.071} & \color{darkred} 0.362 &  72.1 % &  76.3 \scriptsize{(-0.3)} & 80.6 \scriptsize{(+0.4)} 
	\tabularnewline
	Input concat. & 0.079 & \color{darkred} 0.328  & 82.4 % &  77.1 \scriptsize{(+0.4)} &  81.4 \scriptsize{(+1.2)} 
	\tabularnewline
	SemanticGAN  $D_m$ \cite{li2021semantic} & 0.074 & \color{darkred} 0.351 & 83.3 % & 77.2 \scriptsize{(+0.5)} & 81.7 \scriptsize{(+1.5)}
	\tabularnewline
	MCA (ours) & 0.073 & \textbf{0.387} & \textbf{86.6} % & \textbf{77.4} \scriptsize{(+0.7)} & \textbf{82.1} \scriptsize{(+1.9)}
	\tabularnewline
\end{tabular}

\end{minipage}
% -------------------------------------------------------------------
\begin{minipage}{.23\linewidth}



\caption{Ablation on the number of $\mathcal{D}_{\text{low-level}}$ discriminator blocks on DAVIS-17. 
	Bold denotes the best performance.}
\label{table:granularity} %

%\setlength{\tabcolsep}{0.50em}
\renewcommand{\arraystretch}{1.20}
%\centering

%@{\hskip 0.02in}
\centering
\begin{tabular}{@{\hskip 0.03in}c@{\hskip 0.03in}|@{\hskip 0.03in}c@{\hskip 0.03in}|@{\hskip 0.03in}c@{\hskip 0.03in}@{\hskip 0.03in}}
	%& \multicolumn{3}{c||@{\hskip 0.03in}}{\scriptsize \color{black} Synthesis quality} % & \multicolumn{2}{c}{\scriptsize \color{black} Effect on  performance}
	%\tabularnewline		
	
	\multirow{2}{*}{$N_{\text{low-level}}$} & \multirow{2}{*}{SIFID$\downarrow$}  & \multirow{2}{*}{mIoU$_\text{mask}$$\uparrow$} % & \multicolumn{2}{c}{\scriptsize \color{black} of OSVOS \cite{Cae+17}}
	\tabularnewline
	
	& &  % & $\mathcal{J}$ & $\mathcal{F}$ 
	\tabularnewline	
	\hline 	
	
	1 & \color{darkred}0.262\color{black}  & \color{darkred}82.4\color{black}  % & \color{gray} 76.7 \scriptsize{(+0.0)} & \color{gray} 80.2 \scriptsize{(+0.0)} 
	\tabularnewline 
	\arrayrulecolor{lightgray}
	2 & \color{darkred}0.165\color{black}  & \textbf{87.1} % &  76.3 \scriptsize{(-0.3)} & 80.6 \scriptsize{(+0.4)} 
	\tabularnewline
	3 & \color{darkred}0.102\color{black}  & 86.9 % &  77.1 \scriptsize{(+0.4)} &  81.4 \scriptsize{(+1.2)} 
	\tabularnewline
	4 & 0.073 & 86.6 % & 77.2 \scriptsize{(+0.5)} & 81.7 \scriptsize{(+1.5)}
	\tabularnewline
	5 & \textbf{0.070}  & \color{darkred}83.9\color{black} % & \textbf{77.4} \scriptsize{(+0.7)} & \textbf{82.1} \scriptsize{(+1.9)}
	\tabularnewline
\end{tabular}

\end{minipage}








\end{table*}


